Common Problems and Effects of Feedback on Fun When Programming Ozobots in Primary School

Computational thinking is increasingly introduced at primary school level, usually with some form of programming activity. In particular, educational robots provide an opportunity for engaging students with programming through hands-on experiences. However, primary school teachers might not be adequately prepared for teaching computer science related topics, and giving feedback to students can often be challenging: Besides the content of the feedback (e.g., what problems have to be handled), the way the feedback is given is also important, as it can lead to negative emotional effects. To support teachers with the way of giving feedback on common problems when teaching programming with robotics, we conducted a study consisting of seven workshops with three third and four fourth grade primary school classes. Within seven different activities, the 116 primary school children first programmed the Ozobot Evo robot in the pen-and-paper mode and then on a digital device. Throughout these activities we collected data on the problems the students encountered, the feedback given, and the fun they experienced. Our analysis reveals eight categories of problems, which we summarise in this paper together with corresponding possible feedback. We observed that problems that are urgent or can harm the students' self-efficacy have a negative impact on how enjoyable an activity is perceived. While direct instruction significantly decreased the experienced fun, hints had a positive effect. Generally, we found programming the Ozobot Evo to be encouraging for both girls and boys. To support teachers, we discuss ideas for giving encouraging feedback on common problems of Ozobot Evo programming activities and how our findings transfer to other robots.

==> figures/againAgainTable.tex <==
\begin{figure}[tb]
	\centering
	\includegraphics[width=0.5\columnwidth]{grafics/again again table.PNG}
	\vspace{-0.5em}
	\caption{\label{fig:againAgainTable}Again Again table used to measure experienced fun.}
	\vspace{-0.5em}
\end{figure}

==> figures/smileyometer.tex <==
\begin{figure}[tb]
	\includegraphics[width=\columnwidth]{grafics/smileyometer.PNG}
	\vspace{-1.5em}
	\caption{\label{fig:smileyometer}Smileyometer used to measure experienced fun.}
\end{figure}

==> tables/correlationFunFeedback.tex <==
\begin{table}[t]
\centering
\caption{Correlation of interactions and fun measures.}
	\label{tab:correlationFunFeedback}
	%\setlength{\tabcolsep}{0.2em}
	%\resizebox{\columnwidth}{!}{
\begin{tabular}{rrrrrr}

\toprule
 & & \multicolumn{2}{c}{Again Again table} & \multicolumn{2}{c}{Smileyometer} \\
Activity & \#Interactions & $p$ & $r$ & $p$ & $r$ \\

\midrule

1 & \amountFeedbackActivityOne & \correlationAgainTaskOnePValue & \correlationAgainTaskOne & \correlationLikeTaskOnePValue & \correlationLikeTaskOne  \\


2 & \amountFeedbackActivityTwo & \correlationAgainTaskTwoPValue & \correlationAgainTaskTwo & \correlationLikeTaskTwoPValue & \correlationLikeTaskTwo  \\

3 & \amountFeedbackActivityThree & \correlationAgainTaskThreePValue & \correlationAgainTaskThree & \correlationLikeTaskThreePValue & \correlationLikeTaskThree \\

4 & \amountFeedbackActivityFour & \correlationAgainTaskFourPValue & \correlationAgainTaskFour & \correlationLikeTaskFourPValue & \correlationLikeTaskFour  \\

5 & \amountFeedbackActivityFive & \correlationAgainTaskFivePValue & \correlationAgainTaskFive & \correlationLikeTaskFivePValue & \correlationLikeTaskFive  \\

6 & \amountFeedbackActivitySix & \correlationAgainTaskSixPValue & \correlationAgainTaskSix & \correlationLikeTaskSixPValue & \correlationLikeTaskSix  \\

7 & \amountFeedbackActivitySeven & \correlationAgainTaskSevenPValue & \correlationAgainTaskSeven & \correlationLikeTaskSevenPValue & \correlationLikeTaskSeven  \\

all & \amountFeedbackAllActivities & \correlationAllTasksAgain & \correlationAllTasksAgainPValue & \correlationAllTasksLike & \correlationAllTasksLikePValue \\

\bottomrule
\end{tabular}
%}
\end{table}



